A square function involving the center of mass and rectifiability

For a Radon measure $\mu$ on $\mathbb{R}^d$, define $C^n_\mu(x, t)= \ (\frac{1}{t^n} \ |\int_{B(x,t)} \frac{x-y}{t} \, d\mu(y)\ | \ )$. This coefficient quantifies how symmetric the measure $\mu$ is by comparing the center of mass at a given scale and location to the actual center of the ball. We show that if $\mu$ is $n$-rectifiable, then $ \int_0^\infty |C^n_\mu(x,t)|^2 \frac{dt}{t} < \infty \, \, \mu\mbox{-almost everywhere}. $ Together with a previous result of Mayboroda and Volberg, where they showed that the converse holds true, this gives a characterisation of $n$-rectifiability. To prove our main result, we also show that for an $n$-uniformly rectifiable measure, $|C_\mu^n(x,t)|^2 dt/t d\mu$ is a Carleson measure on $\mathrm{spt}(\mu) \times (0,\infty)$. We also show that, whenever a measure $\mu$ is $1$-rectifiable in the plane, then the same Dini condition as above holds for more general kernels. Moreover, we give a characterisation of uniform 1-rectifiability in the plane in terms of a Carleson measure condition.

==> 01intro.tex <==
\section{Introduction}

One of the main object of study of geometric measure theory are rectifiable sets. These are sets that can be covered by Lipschitz images of the euclidean space, up to a set of measure zero. That is:
rectifiable sets (respectively Lipschitz maps) stay at GMT as manifolds (respectively homeomorphisms) stay at differential geometry. 
\begin{definition}
A set $E \subset \R^d$ is called $n$-rectifiable is there exist a countable family of Lipschitz maps $f_k:\R^n \to \R^d$, $k=1,2,...$ such that
\begin{align*}
    \hn \left( E \setminus \bigcup_{k=1}^\infty f_k(\R^n)\right) = 0.
\end{align*}
(Here $\hn$ denotes the $n$-dimensional Hausdorff measure).
\end{definition}
More generally, a \textit{measure} is $n$-rectifiable if there exists an $n$-rectifiable set $E$ and a Borel function $f: \R^d \to \R$ so that $\mu = f \, \hn|_E$.

In this paper, we will move within a smaller category: that of \textit{uniformly rectifiable} (or UR) sets. Uniformly rectifiable sets were firstly introduced by Guy David and Stephen Semmes in \cite{singularintegrals}. We postpone the precise definition to the next section. For now, it is enough to say that uniform rectifiability is a stronger property than rectifiability, since one has control on how much mass in any give ball centered on the set can be covered by just one Lipschitz graph - in contrast to rectifiable sets, where in some places one may need very many graphs to cover just a small portion of the original set.

This sub-area of GMT has very strong ties to fourier analysis. Indeed, not only `\textit{is there an obvious analogy between rectifiability property of sets} (this is GMT) \textit{and differentiability properties of functions}\footnote{We are quoting David and Semmes in \cite{analysisofandon}} (this is Fourier analysis), but also the problems themselves that originally motivated the development of the theory of UR sets. Here's an example.

Consider $f: \R \to \R$ in $L^2(\R)$. Then the following are equivalent (see \cite{stein2}):
\begin{enumerate}
    \item $f$ is locally absolute continuous and $f' \in L^2$. 
    \item $\int_0^\infty \int_\R t^{-2} |f(x+t)+ f(x-t) - 2f(x)|^2 \, dx \frac{dt}{t} < \infty$. 
\end{enumerate}

The quantity  $t^{-1}(f(x+t)+ f(x-t) - 2f(x))$ can be seen as a measurement of how far is $f$ from being affine. With this at hand, the following result by Dorronsoro (\cite{do1}) won't be too surprising. 

\begin{theorem}
	Let $f \in W^{1,2}(\R^d)$ and define
	\begin{align*}
		\Omega_f (x, t) := \left(\inf_A  \frac{1}{t^d}\int_{B(x, t)} \left(\frac{ f(y) - A(y)}{t} \right)^2
		\, dy \right)^{\frac{1}{2}},
	\end{align*}
	where the infimum is taken over all affine functions $A$.
	Then 
	\begin{align*}
		\int_{\R^d} \int_0^\infty \Omega_f(x, t)^2 \, \frac{dt}{t} dx \sim \| \nabla f
		\|_2^2.
	\end{align*}
\end{theorem}

We may naturally (!) consider a similar quantity for sets rather than functions. Take a subset $E \subset \R^n$. Let
\begin{align} \label{eq:01_beta}
\beta_{E, p}^n(x,t):=\inf_L \left(\frac{1}{t^n} \int_{B \cap E} \left(\frac{\dist(y,
L)}{t}\right)^p \, d \hn(y) \right)^{\frac{1}{p}},
\end{align}
Notice the analogy with the quantity $\Omega_f$. In the first case, a quantitative way of answering the question: `If I zoom in on the graph of $f$, does it look flat?' it is proposed; in the second case, a quantitative way of answering to: 'if I zoom in on the set, does it look like a plane?'.

The quantity in \eqref{eq:01_beta} was first introduced by Peter Jones in \cite{jones} as a tool to prove his Analyst's Traveling Salesman theorem (and so it is called Jones-beta number), and further developed by David and Semmes in \cite{singularintegrals}, \cite{analysisofandon}, to show that if a set $E$ is $n$-Ahlfors - David regular (ADR), that is, if there exists a constant $c\geq 1$ such that $c^{-1}\, r^n \hn(B(x, r) \cap E) \leq c \, r^n$ for all $x \in E$, $r>0$, then $E$ is UR if and only if 
\begin{align} \label{eq:01_betacarleson}
    \int_{B_R} \int_0^R \beta_{E, p}^n (x, t)^2 \, \dt \, d \hn|_E(x) \leq C\, R^n.
\end{align}
Moreover, David and Semmes show that a set $E$ is UR if and only if a wide class of Calder\'{o}n-Zygmund kernels are $L^2(E)$ bounded. Indeed, this is precisely the problem which originally motivated David and Semmes: on what sort of sets are Calder\'{o}n - Zygmund kernels $L^2$ bounded?


Recently, another quantity was developed in order to study differentiability properties of functions. In \cite{mateu-verdera}, Roc Alabern, Joan Mateu and Joan Verdera showed that if $f \in W^{1, p}(\R^d)$, then 
\begin{align*}
    \|S(f)\|_p \sim \|\nabla f\|_p,
\end{align*}
where
\begin{align*}
    S(f)^2(x) & := \int_0^\infty \left|\frac{f_{B(x, t)} - f(x)}{t}\right|^2\, \dt \\
    & = \int_0^\infty \left| \frac{1}{|B(x, t)|} \int_{B(x, t)} \frac{f(x)- f(y)}{t} \, dy \, \right|^2 \, \dt.
\end{align*}
Appealing to analogy once more (\textit{`you can prove anything using the Analogy'}\footnote{See U.K. Le Guin, \textit{The Dispossessed}. However, the reader should be warned: analogy can be misleading, see \cite{singularintegrals}, Introduction.}), one may define an analogous quantity for sets, or, more generally for a Radon measure $\mu$ on $\R^d$: we let the $n$-dimensional $C$-number to be defined as
\begin{align*}
    C^n_\mu(x, t) := \left(\frac{1}{t^n} \left|\int \frac{x-y}{t} \, d\mu(y)\right| \right).
\end{align*}

This quantity is not new: Mattila, in \cite{mattila_cauchy}, while investigating for what kind of measures $\mu$ on $\C$ does the Cauchy transform exists $\mu$-almost everywhere (as principal values), gives a complete characterisation of what he call \textit{symmetric} measures, that is, measures that satisfy \begin{align*}
    C_\mu(x, t) = 0 \, \mbox{ for all } x \in \spt(\mu) \mbox{ and for all } t>0.
\end{align*}
He shows that any symmetric locally finite Borel measure on $\C$ is either discrete or coninuous. In the latter case, it is either the $2$-dimensional Lebesgue measure (up to a multiplicative constant) or a countable sum of $1$-dimensional Hausdorff measures restricted to equidistant affine lines. Mattila needed such characterisation to understand the geometry of the tangent measures of a measure $\mu$ for which the Cauchy transform exists $\mu$-almost everywhere, and thus to understand the geometry of $\mu$ itself. 
Briefly after, Mattila and Preiss (see \cite{Mattila-Preiss}) generalised this to the higher dimensional equivalent. They showed that if $\mu$ (a measure in $\R^d$) has lower $n$-dimensional density bounded away from zero and infinity, and if the Riesz transform of $\mu$ exists $\mu$-almost everywhere, then $\mu$ is $n$-rectifiable. Here, too, the authors went to great length in understanding symmetric measures, as they again appear as tangent measures of $\mu$.

We should mention in passing the `sister' theory of \textit{reflectionless} measures, developed by Jaye and Nazarov in \cite{jn1}, \cite{jn2} and \cite{jn3}. In particular, in \cite{jn3}, they provide a new proof of a theorem of Mattila, Melnikov and Verdera (see \cite{mmv}) which states that a $1$-ADR measure $\mu$ whose Cauchy transform is bounded in $L^2(\mu)$, has to be UR. In their proof, showing that an ADR reflectionless measure has to be flat, plays a central role, somehow akin to the role played by Mattila's characterisation of symmetric measures.  

Let $\mu$ be a Radon, $n$-ADR measure. We say that $\mu$ is \textit{quasi-symmetric} if for all balls $B$ centered on $\spt(\mu)$, we have
\begin{align} \label{eq:01_cCarleson}
    \int_{B}\int_0^{r_B} |C_\mu(x, t)|^2 \, \dt\, d\mu(x) \lesssim r_B^n.
\end{align}
Notice that this condition is the same as \eqref{eq:01_betacarleson}, simply applied to a different quantity; it is a common condition in the theory of UR sets and it simply means that $|C_\mu(x, t)|^2 \dt \, d\mu$ is a Carleson measure on $\spt(\mu)\times (0, \infty)$.
We call ADR measures satisfying \eqref{eq:01_cCarleson} quasi-symmetric because they must have very small $C_\mu$ numbers at small scales, that is, they must be very close to being symmetric. 

The main result of this paper is the following. 
\begin{theorem} \label{main}
Let $\mu$ be an $n$-ADR measure on $\R^d$. Then $\mu$ is $n$-uniformly rectifiable if and only if it is quasi-symmetric.
\end{theorem}

\textbf{Plan of the paper.}
The first section below is devoted to the collection of some relevant results and definitions from the literature. The subsequent two sections are devoted to proving Theorem \ref{main} for a certain smoothed version of the $C_\mu$ numbers. The results obtained there will then be used in the last two section to prove Theorem \ref{main}. Throughout the paper, we have especially used tools and strategies originated in the works of Tolsa and Mas \cite{mastolsa} and \cite{mastolsa2}, and further developed by Tolsa in \cite{tolsa2008} and by Chousionis, Garnett, Le and Tolsa in \cite{tolsa2014}.

\subsection{Acknowledgments}
I would like to thank Jonas Azzam, my supervisor; his help and patience have been indispensable to make any progress in this work. I also thank Raanan Schul and Xavier Tolsa for useful discussions.





==> 05ns_c_ur.tex <==
\section{Non smooth case: Carleson condition implies uniform rectifiability} \label{section:ns_carl_ur}

This section will be devoted to prove the following proposition. 

\begin{proposition} \label{proposition:ns_c_ur}
Let $\mu$ be an $n$-AD-regular measure on $\R^d$. If, for all balls $B$ centered on $\spt(\mu)$, 
\begin{align*}
\int_B \int_0^{r_B} \left| C_\mu(x,t)\right|^2 \, \dt \, d\mu(x) \lesssim r_B^n,
\end{align*}
then $\mu$ is $n$-uniformly rectifiable.
\end{proposition}

We will prove Proposition \ref{proposition:ns_c_ur} through the following lemma. 

\begin{lemma} \label{lemma:convexcomb}
Let $\phi$ be as in Definition \ref{def:smoothed_c}. Then 
\begin{align*}
    \int_0^\infty |\cmufi(x,t)|^2 \, \dt \lesssim \int_0^\infty |C_\mu(x,t)|^2\, \dt.
\end{align*}
\end{lemma}

\begin{remark}
Notice that, assuming that Lemma \ref{lemma:convexcomb} holds, Proposition \ref{proposition:ns_c_ur} follows immediately, since 
\begin{align*}
    \int_B \int_0^{r_B} \left| \cmufi(x,t)\right|^2 \, \dt \, d\mu(x) \lesssim \int_B \int_0^{r_B} \left| C_\mu(x,t)\right|^2 \, \dt \, d\mu(x) \lesssim r_B^n.
\end{align*}
Hence we may apply Proposition \ref{proposition:smooth_c_ur}.
\end{remark}

\begin{proof}[Proof of Lemma \ref{lemma:convexcomb}]
For our purposes here, it is enough to let $N$ in equation \eqref{eq:02_30} (where $\phi$ is defined) to be equal to $1$. We use a trick from, once again, \cite{tolsa2014}; see pages 13 and 14. We set 
\begin{align} \label{eq:ns_c_urL1}
    \phi_t(s)= \frac{1}{t^n} \exp\left(-\frac{s^2}{t^2}\right) = \int_0^\infty \chara_{[0,r]}(s)\,  r^{-n} \tilde \phi(r) \, dr = \int_s^\infty r^{-n} \tilde \phi(r)\, dr.
\end{align}
and we want to solve for $\tilde \phi$. We differentiate with respect to $s$ equation \eqref{eq:ns_c_urL1}:
\begin{align*}
-\frac{2s}{t^{n+2}} \exp\left(-\frac{s^2}{t^2}\right) = - \tilde \phi(s)s^{-n}.
\end{align*}
Thus 
\begin{align*}
    \tilde \phi(s) = \tilde \phi_t(s) = \frac{2 s^{n+1}}{t^{n+2}} \exp\left(-\frac{s^2}{t^2}\right).
\end{align*}
Then we write
\begin{align} \label{eq:ns_c_urL2}
    & \int_0^\infty \left| \cmufi (x,t) \right|^2 \, \dt \\
    & = \int_0^\infty \left| \int \quotyx \phi_t(x-y) \, d\mu(y) \right|^2 \, \dt \nonumber \\
    & = \int_0^\infty \left| \int_{\R^d} \quotyx \left(\int_0^\infty \chara_{[0,r]}(|x-y|) r^{-n} \tilde \phi_t(r) \, dr \right) \, d\mu(y) \right|^2 \, \dt \nonumber \\
    & = \int_0^\infty \left| \int_0^\infty   \frac{r}{t}\, \tilde\phi_t(r) \left(r^{-n} \int_{\R^d} \ps{\frac{x-y}{r}} \,  \chara_{[0,r]}(|x-y|)  \,d\mu(y) \right) \,  dr   \right|^2 \, \dt \nonumber \\
    & = \int_0^\infty \left| \int_0^\infty  \frac{r}{t} \tilde \phi_t(r) \, C_\mu(x,r) \, dr\right|^2 \dt \nonumber \\
    & \leq \int_0^\infty \int_0^\infty \left|  \frac{r}{t} \tilde\phi_t(r)\right|^2 |C_\mu(x,r)|^2 \, dr \, \dt.
\end{align}
Thus 
\begin{align*}
    \eqref{eq:ns_c_urL2} & \lesssim_n \int_0^\infty \int_0^\infty  \frac{r}{t} \tilde \phi(r) |C_\mu(x,r)|^2 \, dr \, \dt 
    & = \int_0^\infty |C_\mu(x,r)|^2 \, \left( \int_0^\infty \frac{r}{t} \tilde \phi_t(r) \dt\right) \,dr.
\end{align*}
We see that, through a change of variables,
\begin{align*}
    \int_0^\infty \frac{r}{t} \tilde \phi_t(r) \dt & = 2 \int_0^\infty \frac{r^{n+2}}{t^{n+2}} \exp\left(-\frac{r^2}{t^2}\right) \, \frac{dt}{t^2}\\
    & = \frac{2}{r} \int_0^\infty s^{n+2} \exp\left(-s^2\right)\, ds \\
    & \lesssim \frac{1}{r}.
\end{align*}
Hence we obtain
\begin{align*}
    \int_0^\infty \left| \cmufi (x,t) \right|^2 \, \dt \lesssim \int_0^\infty \left| C_\mu(x,r)\right|^2 \, \frac{dr}{r}.
\end{align*}
\end{proof}
